Near-Optimal Correlation Clustering with Privacy

Correlation clustering is a central problem in unsupervised learning, with applications spanning community detection, duplicate detection, automated labelling and many more. In the correlation clustering problem one receives as input a set of nodes and for each node a list of co-clustering preferences, and the goal is to output a clustering that minimizes the disagreement with the specified nodes' preferences. In this paper, we introduce a simple and computationally efficient algorithm for the correlation clustering problem with provable privacy guarantees. Our approximation guarantees are stronger than those shown in prior work and are optimal up to logarithmic factors.

==> 600-mpc-implementation.tex <==
\section{MPC implementation}
\label{sec:mpc_implementation}

In this section we show how to implement \cref{alg:main} in the MPC model using only $O(1)$ parallel rounds. Our algorithm requires $n^{\mu}$ memory per machine, and a total of $O(|E^{+}| \log n)$ memory over all machines. 
Our implementation closely follows the one by \cite{cohen2021correlation}.
%Hence, we only describe the necessary adjustments to the algorithm to achieve our goal.

\paragraph{Computing Noised Agreements.}
Given that we cannot compute $|N(u) \triangle N(v)|$ for all edges $\{u,v\} \in E^{+}$ efficiently in MPC using only $\widetilde{O}(|E^{+}|)$ memory, we are going to approximate the value of $|N(u) \triangle N(v)|$ for all edges $\{u,v\} \in E^{+}$ using samples of $N(u), N(v)$. This procedure has been described in \cite{cohen2021correlation}, but we repeat it here for completeness.

First, notice that we only need to compute $|N(u) \triangle N(v)|$ for the edges $\{u,v\} \in E^{+}$ such that $|d(u) - d(v)| < \beta \cdot \max(d(u), d(v)) - \cE_{u,v}$, as otherwise $u,v$ cannot be in noised agreement.
Let $\hat{\beta} = 11\beta/10$.
We create $t=O(\log n / \hat{\beta})$ samples $S(1), \dots, S(t)$ of $V$, where node $v$ is part of sample $S(j)$ with probability $\min(\frac{a \log n}{ \hat{\beta} \cdot j}, 1)$, where $a$ is a large-enough constant that we will fix later.
For each vertex $v\in V$, we set $S(v,j)=S(j)\cap N(v)$, and let $j_v$ be the largest power of $1 / (1 - \hat{\beta})$ smaller or equal than $d(v)$. 
These sets are used to estimate $|N(u) \triangle N(v)|$.
For each vertex $v \in V$, we only need to keep $S(v,j_v)$ and $S(v, j_v/(1-\hat{\beta}))$, as we only need to estimate $|N(u) \triangle N(v)|$ for the pairs $u,v$ for which $|d(u) - d(v)| < \beta \cdot \max(d(u), d(v)) - \cE_{u,v} < \hat{\beta}\cdot \max(d(u), d(v))$, where the last inequality follows by a simple application of Chernoff bound.
For each edge $\{u,v\}$ we chose $j$ to be either $j = j_u = j_v$, $j = j_u = j_v / (1-\hat{\beta})$, or $j = j_v = j_u / (1-\hat{\beta})$, depending on which of the three equalities hold. We define the variable $X_{u,v}$ to be equal to $|S(u,j) \triangle S(v,j)|$. As shown in
\cite{cohen2021correlation}, if $\frac{a \log{n}}{\hat{\beta} \cdot j}\geq 1$ then $X_{u,v} = |N(u) \triangle N(v)|$, and otherwise, it holds that $\E{X_{u,v}} = \frac{\alpha\cdot \log{n}}{\hat{\beta} \cdot j}|N(u) \triangle N(v)|$. 
%That is, if two vertices $u,v$ are in agreement then it holds that 
% \[
%     \E{X_{u, v}} \le \frac{a \cdot \log{n}}{\beta \cdot j} \cdot \beta \cdot \max(d(u), d(v))
%     = \frac{a \cdot \log{n}}{j} \cdot \max(d(u), d(v)).
% \]

By linearity of expectation, if $\frac{a \log{n}}{\hat{\beta} \cdot j}< 1$, for a fixed $\cE_{u,v}$, we have that 
\[
\E{X_{u,v} + \frac{\alpha\cdot \log{n}}{\hat{\beta} \cdot j} \cdot \cE_{u,v}} 
= \frac{\alpha\cdot \log{n}}{\hat{\beta} \cdot j} \left(|N(u) \triangle N(v)| + \cE_{u,v}\right)
\]

We use $X_{u,v}$ to compute noised agreement as described in \cref{alg:noised-agreement} by observing that if two vertices $u,v$ are in noised agreement, then we have that
\begin{align*}
    \E{X_{u,v}} + \frac{\alpha\cdot \log{n}}{\hat{\beta} \cdot j} \cdot \cE_{u,v} 
    & \le \frac{a \cdot \log{n}}{\hat{\beta} \cdot j} \cdot \hat{\beta} \cdot \max(d(u), d(v))
    \\ & = \frac{a \cdot \log{n}}{j} \cdot \max(d(u), d(v))
\end{align*}

For the details on how to efficiently compute $X_{u,v}$ for each $\{u,v\}\in E^{+}$ using $O(1)$ MPC rounds and only $O(n^{\mu})$ memory, for any $\mu > 0$, we refer the interested reader to \cite{cohen2021correlation}.

\begin{algorithm2e}
\LinesNumbered
%   \Input{$G=(V,E)$: a graph \\
% 		$\eps$, $\delta$: privacy parameters}
% 		%\\		$\beta$, $\lambda$: approximation-related parameters}
	If $|d(u) - d(v)| \geq \beta \cdot \max(d(u), d(v)) - \cE_{u,v}$ return ``no''.
    % If $d(u)$ and $d(v)$ are not within factor $(1-\beta)$ return ``no''. \Nnote{TODO: adjust and explain this.}
    
    $\tau \gets \frac{a \cdot \log{n}}{j} \cdot \left(\max(d(u), d(v)) - \frac{\cE_{u,v}}{\hat{\beta}} \right)$

    If $X_{u, v} \le 0.9 \cdot \tau$, then return ``yes''. Otherwise, return ``no''.
    \label{line:mpc-noised-agreement-threshold}
  \caption{Decides whether $u$ and $v$ are in noised agreement}
	\label{alg:noised-agreement}
\end{algorithm2e}

\begin{restatable}{lemma}{noisedagreement} 
% \begin{lemma}
\label{lemma:MPC-noised-agreement}
For any constant $\mu > 0$, there exists an MPC $(2.9 \epsagr, 2.4 \deltagr)$-DP algorithm that, given a signed graph $G = (V, E^+)$, in $O(1)$ rounds for all pairs of vertices $\{u, v\} \in E^+$ outputs ``Yes'' if $u$ and $v$ are in $0.8$-noised agreement, and outputs ``No'' if $u$ and $v$ are not in noised agreement. Letting $n = |V|$, this algorithm succeeds with probability $1 - 1/n$, uses $n^{\mu}$ memory per machine, and uses a total memory of $\tilde{O}(|E^+|)$.
% \end{lemma}
\end{restatable}

\paragraph{Computing the connected components of $\hat{G}$.} 
\cite{cohen2021correlation} described a simple $O(1)$-round MPC algorithm for computing the connected components of a graph with constant diameter.
We can use this to compute the connected components of $\hat{G}$ (in  \cref{line:component} of \cref{alg:main}) as implied by the following lemma.

% \begin{lemma}
\begin{restatable}{lemma}{lowdiameteringraph} 
\label{lemma:low-diameter-graph}
For $\beta, \lambda$ such that $\beta \cdot 5 + \lambda \cdot 2 < 1/1.1$, it holds that $\hat{G}$ has diameter $4$. 
% \end{lemma}
\end{restatable}

Hence, we have the following Lemma.
\begin{lemma}
\label{lemma:mpc-components}
For any constant $\mu > 0$, there exists an MPC algorithm that computes the connected component of $\hat{G}$ in \cref{line:component} of \cref{alg:main} in $O(1)$ rounds. Letting $n=|V|$, the algorithm used $n^{\mu}$ memory per machine, and $\tilde{O}(|E^{+}|)$ total memory over all machines.
\end{lemma}

\paragraph{Approximation Analysis.}

\begin{restatable}{theorem}{mpcmainresult} 
% \begin{theorem}
\label{theorem:MPC-main}
	For any constant $\mu> 0$, there exists an MPC algorithm that, given a signed graph $G = (V, E^+)$, where $E^+$ denotes the set of edges with weight +1, in $O(1)$ rounds computes a $O(1)$-approximate $(\epsilon, \delta)$-DP correlation clustering. Letting $n = |V|$, this algorithm succeeds with probability at least $1-1/n$ and requires $O(n^{\mu})$ memory per machine. Moreover, the algorithm uses a total memory of $O(|E^+| \cdot \log{n})$.
% \end{theorem}
\end{restatable}

